An MCMC Method for Uncertainty Set Generation via Operator-Theoretic Metrics

Model uncertainty sets are required in many robust optimization problems, such as robust control and prediction with uncertainty, but there is no definite methodology to generate uncertainty sets for nonlinear dynamical systems. In this paper, we propose a method for model uncertainty set generation via Markov chain Monte Carlo. The proposed method samples from distributions over dynamical systems via metrics over transfer operators and is applicable to general nonlinear systems. We adapt Hamiltonian Monte Carlo for sampling high-dimensional transfer operators in a computationally efficient manner. We present numerical examples to validate the proposed method for uncertainty set generation.

==> _note_projection_kernel.tex <==
\subsection{Projection kernel and gradients}

% [De Cock and De Moor, S&C Letters, 2002] K. De Cock and B. De Moor, “Subspace angles between ARMA models,” Systems & Control Letters, vol. 46, no. 4, pp. 265–270, 2002.

% [Ishikawa+, NeurIPS, 2018] I. Ishikawa, K. Fujii, M. Ikeda, Y. Hashimoto, and Y. Kawahara, “Metric on nonlinear dynamical systems with Perron--Frobenius operators,” in Advances in Neural Information Processing Systems 31, 2018, pp. 2856–2866.

% [Huang+, NeurIPS, 2017] W. Huang, M. Harandi, T. Zhang, L. Fan, F. Sun, and J. Huang, “Efficient optimization for linear dynamical systems with applications to clustering and sparse coding,” in Advances in Neural Information Processing Systems 30, 2017, pp. 3444–3454.

Consider two linear dynamical systems
\begin{equation*}
    \bm{x}^{(1)}_{t+1} = \bm{A}_1 \bm{x}^{(1)}_t
    \quad\text{and}\quad
    \bm{x}^{(2)}_{t+1} = \bm{A}_2 \bm{x}^{(2)}_t,
\end{equation*}
where $\bm{x}^{(i)} \in \mathbb{R}^p$ and $\bm{A}_i \in \mathbb{R}^{p \times p}$ for $i=1,2$.
Here we have to assume that $\bm{A}_i$ is stable, i.e., $\rho(\bm{A}_i)<1$, which may limit the usefulness of the discussion below, though.

Let $\bm{O}_i$ be the extended observability matrix corresponding to $\bm{A}_i$, i.e.,
\begin{equation*}
    \bm{O}_i = \begin{bmatrix} \bm{I} & \bm{A}_i & \bm{A}_i^2 & \cdots \end{bmatrix}^\tr.
\end{equation*}
The projection kernel, which can be used to construct a metric based on the subspace angles between the column spaces of $\bm{O}_1$ and $\bm{O}_2$, is defined as
\begin{equation*}
    k_\text{proj} (\bm{A}_1,\bm{A}_2)
    = \operatorname{trace} ( \bm{P}_1 \bm{P}_2 )
    = \operatorname{trace} \Big ( \big( \bm{O}_1^\tr \bm{O}_1 \big)^{-1} \bm{O}_1^\tr \bm{O}_2 \big( \bm{O}_2^\tr \bm{O}_2 \big)^{-1} \bm{O}_2^\tr \bm{O}_1 \Big),
\end{equation*}
where $P_i$ denotes the orthogonal projection matrix onto the column space of $\bm{O}_i$.
A corresponding metric can be constructed as $d_\text{proj}^2 (\bm{A}_1, \bm{A}_2) = 1 - k^2_\text{proj} (\bm{A}_1, \bm{A}_2) / p^2$, where we use the fact $k_\text{proj}(\bm{A}_i, \bm{A}_i)=p$.
Then, based on this $d_\text{proj}$, we can compute the regularization term.

Then how can we actually compute the values of $k_\text{proj}$ and their gradients?
It is known that a matrix $\bm{G}_{i,j} = \bm{O}_i^\tr \bm{O}_j$ for $i,j=\{1,2\}$ can be computed by solving a Sylvester equation:
\begin{equation*}
    \bm{A}_i^\tr \bm{G}_{i,j} \bm{A}_j - \bm{G}_{i,j} + \bm{I} = \bm{0}.
\end{equation*}
Using the solutions of such Sylvester equations, we can compute the values of $k_\text{proj}$.
As for the gradients, from Theorem 4 in [Huang+, NeurIPS, 2017], we have
\begin{equation*}\begin{aligned}
    \frac{\partial k_\text{proj}(\bm{A}_i,\bm{A}_j)}{\partial \bm{A}_i} &= \bm{G}_{i,j} \bm{A}_j \bm{R}_{i,j}^\tr + 2 \bm{G}_{i,i} \bm{A}_i \bm{R}_{i,i}^\tr,
    \quad\text{and}\
    \\
    \frac{\partial k_\text{proj}(\bm{A}_i,\bm{A}_j)}{\partial \bm{A}_j} &= \bm{G}_{i,j}^\tr \bm{A}_i \bm{R}_{i,j} + 2 \bm{G}_{j,j}^\tr \bm{A}_j \bm{R}_{j,j},
\end{aligned}\end{equation*}
where $\bm{R}_{i,j}$ is computed by solving another Sylvester equation:
\begin{equation*}
    \bm{A}_i \bm{R}_{i,j} \bm{A}_j^\tr - \bm{R}_{i,j} + \frac{\partial k_\text{proj}(\bm{A}_i,\bm{A}_j)}{\partial \bm{G}_{i,j}} = \bm{0}.
\end{equation*}
Here,
\begin{equation*}\begin{aligned}
    \frac{\partial k_\text{proj}(\bm{A}_i,\bm{A}_j)}{\partial \bm{G}_{i,j}} &= 2 \bm{G}_{i,i}^{-1} \bm{G}_{i,j} \bm{G}_{j,j}^{-1},
    \quad\text{and}
    \\
    \frac{\partial k_\text{proj}(\bm{A}_i,\bm{A}_j)}{\partial \bm{G}_{i,i}} &= - \bm{G}_{i,i}^{-1} \bm{G}_{i,j} \bm{G}_{j,j}^{-1} \bm{G}_{i,j}^\tr \bm{G}_{i,i}^{-1}.
\end{aligned}\end{equation*}

Note that solving a Sylvester equation requires $O(p^3)$ flops.
When $p$ is too large, which would not be the case basically, we may have to conduct dimensionality reduction of data as preprocessing.

\textcolor{red}{IMPORTANT NOTE.}
The above discussion is for stable linear dynamics.
Thus, basically, it cannot be applied to the case with Koopman operators (maybe).
As for the Koopman operator, [Ishikawa+, NeurIPS, 2018] proposed a similar kernel and associated metric, but it has to be evaluated using trajectories from dynamics.
And in fact, it coincides with the kernel proposed by [De Cock and De Moor, S\&C Letters, 2002], which is basically the same with the projection kernel above, if the dynamics are linear and stable.
